Single Stage Class Agnostic Common Object Detection: A Simple Baseline

This paper addresses the problem of common object detection, which aims to detect objects of similar categories from a set of images. Although it shares some similarities with the standard object detection and co-segmentation, common object detection, recently promoted by \cite{Jiang2019a}, has some unique advantages and challenges. First, it is designed to work on both closed-set and open-set conditions, a.k.a. known and unknown objects. Second, it must be able to match objects of the same category but not restricted to the same instance, texture, or posture. Third, it can distinguish multiple objects. In this work, we introduce the Single Stage Common Object Detection (SSCOD) to detect class-agnostic common objects from an image set. The proposed method is built upon the standard single-stage object detector. Furthermore, an embedded branch is introduced to generate the object's representation feature, and their similarity is measured by cosine distance. Experiments are conducted on PASCAL VOC 2007 and COCO 2014 datasets. While being simple and flexible, our proposed SSCOD built upon ATSSNet performs significantly better than the baseline of the standard object detection, while still be able to match objects of unknown categories. Our source code can be found at \href{https://github.com/cybercore-co-ltd/Single-Stage-Common-Object-Detection}{(URL)}

==> Tex/SelfDevelop_CoDet.tex <==
\subsection{Paper summary}
The paper \cite{Jiang2019} performs common object detection (co-detection) in form of bounding box, which is easier to obtain than the label of Co-Segmentation. The core idea of co-detection and co-segmentation is similar. During training, we impose the constraint that the features of the same class (positive pairs) have high correlation, while that of different classes (negative pairs) has low correlation. The difference are that:
\begin{itemize}
	\item Co-segmentation perform at the pixel level, and thus harder to separate different instance. In contrast, Co-Detection compares the similarity between bounding boxes, thus natively supports multiple object detection. In short, Co-segmentation at instance level follows "Bottom-Up" approach, while Co-detection follows "top-down" approach, thus it is simpler.
	\item Another advantage is that co-detection is easily incorporated to any base-line Object Detection, such as Faster-RCNN. In addition, co-detection can be leveraged to Co-segmentation, by adding a segmentation mask head to the network, as done in the renown work Mask-RCNN.
\end{itemize}

The solution is based on two stage detector Faster RCNN [2], but take pair images as the input. The first stage RPN will output the proposal lists and correspond annotation labels to generate pair features set. These pairs are assigned to positive pairs if they stem from the same class, the opposite was true for negative pairs, which form of two disparate class proposals.

Pair images after separate is pass into two heads called Matching modules. The first one use Siamese [3] method to generate two embedding features and then compare the cosine distance from these features to determine whether it is similar object or not, the second module was called Relation Matching, which take the concatenate feature of a pair to convolution modules and then output a score in range 0 and 1. Both of Siamese score and relation score will be used in the test phase to pick up the top final output bounding box results.

The paper pipeline is illustrated in \fig{CommonDetect}

\begin{figure}[!h]
	\centering
	\begin{subfigure}{0.4\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./Fig/ClassAgnostic_output.png}	
		\caption{Expected Input-Output }
	\end{subfigure}%
	~
	\begin{subfigure}{.6\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./Fig/ClassAgnostic.png}
		\caption{Solution Pipeline.}
		
	\end{subfigure}
	\caption{Class Agnostic Common Object Detection. Reprinted from \cite{Jiang2019}}
	\label{fig:CommonDetect}
\end{figure}

\subsection{Reproducing the paper}
In our implementation, as the base-line, we try to reproduce the results from the paper. Specifically, we take the output from Faster-RCNN 's proposal head with ResNet50 as backbone to perform matching. The code is implemented based on mmdetection. Only simple flip image is used for data augmentation, and SGD is used for optimizer.

\subsubsection{Dataset Generation}
As the paper described, dataset was used is pair images generating from VOC and COCO popular object detection datasets. Below is the pseudo code to create our dataset offline:
\begin{center}
\noindent\fbox{%	
\begin{minipage}{\dimexpr0.8\linewidth \fboxsep-2\fboxrule\relax}
\begin{algorithm}[H]
	\KwData{Dataset $\D$ with Annotation $\textbf{A}$}
	\KwResult{List of pair of images that share common class Pair\_List\_total  }
	\textbf{Initialization}\: Pair\_List\_total=[], L = len($\D$)
	
	\For{i from 0 to L-1 }{
		\For{j from (i+1) to L]}{
			\If{set($\textbf{A}$[i]) $\cap$ set($\textbf{A}$[j]) $\neq$ $\emptyset$}{
				Pair\_List\_total.append([i,j])	
			}
		}
	}
	\textbf{During training}: Sample a subset number of image pairs from Pair\_List\_total
	\caption{Create List of Image Pair Off-line}
\end{algorithm}
\end{minipage}% 
}
\end{center}

The advantages of this approach is that we generate the pair offline, hence, during training we can randomly pickup a pair of images for training so that dataloading is faster. The disadvantage is that if there are many categories in an image, there are huge number of pairs, which cause memory issue. Thus, we can randomly pick up a subset from the pair list total. This creates consistent dataset during training and faster speed. Below is the general information of number pairs:
\begin{itemize}
	\item VOC 2007 dataset: using 5000 images generates 67200 pairs list.
	\item COCO 2017 dataset: using 10000 images generates approximately 100000 pairs list
\end{itemize}

\subsubsection{Training configuration and parameter setting}
The configuration for training is followed Faster-RCNN configuration, which use backbone Resnet50 and FPN to extract feature for RPN network. The training start with loading pre-trained weight from COCO, the number epoch was set to 15 with multi-step learing rate policy. The setting for region proposal network was slightly changed:
\begin{itemize}
	\item For VOC dataset, the maximum of proposal list is set to 128. 
	\item For CoCo dataset, the maximum of proposal list is set to 64. In our experience, selecting many proposals yield worse results. The reason may be that CoCo has much more number of object categories, and select a large number of proposal can leads to large number of categories trying to optimizing at once.
\end{itemize}

The final score is calculated as: 
\begin{equation}
Score = p_1 \times p_2 \times Sim(P1,P2)^{1/2}
\end{equation}
where $p_1, p_2$ are the confidence score of Proposal 1 and 2 to be object (foreground), and $Sim(P1,P2)$ is their similarity score (Either relationship or Siamese score).   

\subsubsection{Testing and Evaluation Results}
To evaluate the performance of Co-detection, the common metric mAP is not suitable for this task, as we perform class-agnostic detection between image pair. According to the paper, a true-positive common object pair must satisfy:
\begin{itemize}
	\item The IoU of detected boxes with ground-truth boxes of each image need to greater than a threshold.
	\item The ground-truth boxes matched with this pair belong to the same category. 
\end{itemize}

For simplicity, we evaluate based on Recall and Precision values at different IoU threshold only. \Tab{CoDetEval} shows our experiments results. 

\begin{table}[h!]
	\centering
	\caption{Recall and Precision scores evaluated at differen IoU threshold}
	\label{Tab:CoDetEval}
	\begin{tabular}{|l|l|l|l|l|}
		\hline
		\multirow{2}{*}{Dataset}   & \multirow{2}{*}{Matching Module} & \multicolumn{3}{c|}{Recall / Precision}                             \\ \cline{3-5} 
		&                                  & IoU \textgreater 0.5 & IoU \textgreater 0.6 & IoU \textgreater{}0.7 \\ \hline
		\multirow{2}{*}{VOC Test}  & Siamese                          & 0.8420 / 0.0346      & 0.8350 / 0.0343      & 0.877 / 0.036         \\ \cline{2-5} 
		& Relation                         & 0.8830 / 0.0344      & 0.8270 / 0.0340      & 0.867 / 0.0356        \\ \hline
		\multirow{2}{*}{CoCo Test} & Siamese                          & 0.1280 / 0.0874      & 0.1190 / 0.0768      & 0.1444 / 0.0933       \\ \cline{2-5} 
		& Relation                         & 0.1748 / 0.1129      & 0.1852 / 0.1196      & 0.2087 / 0.1348       \\ \hline
	\end{tabular}
\end{table}
\subsubsection{Visualize Inference Results}
We inspect the results using images containing single objects only. This setting is also used in the paper \cite{Jiang2019}. The results are shown in \fig{CoDetSingleInfer}
To perform co-detection using the video from Shinkansen dataset, we tested using two ways to create an image pair:
\begin{itemize}
	\item using frame $t$ and frame $t-1$. 
	\item using frame $t$ and its horizontal flip. 
\end{itemize}

\Fig{CoDetShinkansen} shows some results by using image pair (t,t-1).
\Fig{CoDetResult} and \Fig{CoDetResult_2} shows comparing results between the two of testing algorithm on the video dataset. In general, the algorithm works and can detect common object, which is denoted by same color. However, the results are still noisy. The case using flip image yield better results, as it can also detect small items, such as "phone" and "picture frame", although these classes are not used in train dataset.  

\subsubsection{Problem and Difficulties} 
Even the method that the author proposed was clear and understandable, there are some difficulties and issues that we encountered when re-implemented this paper.
\begin{itemize}
	\item The detail description in paper is not adequate to refer parameter setting exactly.
	\item The way dataset is created and sampling is insufficient. 
	\item The paper shows the final test with images in simple scenario, such as containing only single object. Also, in their paper, they show some failure case for complex background. This is questioning if the method can work in our Shinkansen dataset.
\end{itemize}

\subsection{Proposed solution to improve}
In the first version, we created a fixed number of image pairs offline. During trainig, we consider the common objects in each pair only without considering that they possibly share some common objects with other pairs in a training batch. This hence does not utilize all possible matching pair at one iteration.

To address this problem, we proposed an update version, where we create a dataset as follow:

\begin{center}
	\noindent\fbox{%	
		\begin{minipage}{\dimexpr 0.9\linewidth \fboxsep-2\fboxrule\relax}
			\begin{algorithm}[H]
				\KwData{Dataset $\D$ with Annotation $\textbf{A}$}
				\KwResult{Dictionary collecting all imgID of each class: ID\_Dict \textbf{T}}
				\textbf{Initialization}: \textbf{T}=dict(Class\_i:[] for i from 1 to L), L = len($\D$)
							
				\For{i in range(0,L)}{					
					class\_set = Set($\textbf{A}$[i]) \tcp*{Find all unique classes in img[i]}					
					\For {class\_j in class\_set}{
						\textbf{T}['class\_j'].append(imgID[i]) \tcp*{ Add ID of img[i] to the class}
					} 
				}
				
				\caption{Create Dictionary to collect ImageID for each class}
			\end{algorithm}
		\end{minipage}% 
	}
\end{center}  

From the ID\_Dict, we select the class that has most images as the base class. During training, we sample the data in a batch as follow:
 
\begin{center}
	\noindent\fbox{%	
		\begin{minipage}{\dimexpr 0.9\linewidth \fboxsep-2\fboxrule\relax}
			\begin{algorithm}[H]
				\KwData{Dataset $\D$ with Annotation $\textbf{A}$, ID\_Dict \textbf{T}, base class $b$, batch size N }
				\KwResult{ Batch data}
				\textbf{Initialization}: Batch\_data=[]
				
				\For{i in range(0,N)}{
					- Random sample an image $I_1$ from the base class $b$: $I_1=rand(T[`b`])$)\\
					- Random sample a class $c$ appearing in $I_1$ except the base class $c \neq b$ \\
					- Random sample an image $I_2$ from the class $c$: $I_2=rand(T[`c`])$) \\
					- \If {$I_1 \neq I_2$}{ Batch\_data.append[$[I_1,I_2]$)	}						
				}			
				\caption{Sampling Strategy for CoDet algorithm}
			\end{algorithm}
		\end{minipage}% 
	}
\end{center}

\begin{itemize}
	\item Sampling in this way ensure that all samples in the batch share at least the base class. In addition, image pair in each row shares another class.
	\item During training, we compute matching loss across all proposals. For instance, if we have total $N$ proposal, we then have $N(N-1)/2$ number of matching pairs, both positive and negatives.
	\item Due to the possible imbalance between the number of positive and negative pairs, we use Focal Loss instead of their proposed Cross Entropy.
\end{itemize}
 


%	\vspace{0.5in}
%	\begin{subfigure}{.9\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{./Fig/CoDet_flip/20200227_021324_050708294_4_flip.jpg}	
%		\includegraphics[width=\textwidth]{./Fig/CoDet_flip/20200227_021324_050708294_10_flip.jpg}
%		\caption{Using frame $t$ and its horizontal flip}
%	\end{subfigure}
%	\caption{Detection results of Class Agnostic Common Object Detection.}
%	\label{fig:CoDetResult_2}


	

==> Tex/review_obj_detection.tex <==
\subsubsection{Overview}  
Comparing to image classification for a single object, object detection is much more challenging since it has to perform not only object localization and classification simultaneously, but also for multiple objects. This leads to complicated structure and pipeline, which in our opinion can divide into 5 orthogonal sub-modules, namely: \textbf{framework, backbone, neck, head} and \textbf{loss functions}.

Common Object Detection framework can be separated into two main approaches, namely two stages and one stage approach, each aims for different compromission between accuracy and speed.
\begin{itemize}
	\item Mile-stone works in two stage approach can be named as Regional-based convolutional neural network (R-CNN) \cite{Girshick2014}, Fast R-CNN \cite{girshick2015fast}, Faster R-CNN \cite{Ren2015} and Mask R-CNN \cite{He2017a}. This approach is based on a backbone CNN to extract features, which is then attached to two CNN modules: (1) the first one proposes possible regions containing objects, a.k.a anchors, and (2) the second module contains two sub-nets: a classification head to classify the object and a regression head to predict bounding boxes offset from anchor. 

	Since Region Proposal is the core component, recent works, such as RPN \cite{shaoqingrpn} and Iterative RPN \cite{spyrosgidarisrpn}, attempt to enhance its performance. Particularly, Cascade RPN \cite{thangvurpn} improves the quality of region proposal by using Adaptive Convolution and combine anchor-based and anchor-free criteria to define positive boxes. In general, two-stage approaches yields higher accuracy but at slower speed due to its complex structure.

	\item The one stage methods were developed later to improve speed, and the representative works are Single Shot MultiBox Detector (SSD) \cite{Liu2016} family, You-Only-Look-Once (YOLO)\cite{Redmon2017, Redmon2018}, and RetinaNet \cite{Lin}. The key advantage of this approach is to omit the proposal region step but instead use sliding-window principle. Specifically, at each cell in a feature map, a set of default anchors with different scales and ratios  are predefined, and marked as positive if it is highly overlap with ground-truth box, otherwise negative. The second step will then perform classification and bounding box regression on each anchor similar to the two-stage approach.
\end{itemize}

Recently, the separation between these two frameworks gradually becomes less and less clear as they tend to borrow the ideas of each other. In principle, except the difference on using only a small proposed set of anchor boxes (two-stage) or all prior-box (one-stage), the modern Object Detection framework consists of following main modules:
\begin{itemize}
	\item \textbf{Anchor Box} is to define the based-ground for bounding box regression, which separates the areas containing objects from background during training. 
	\item \textbf{Backbone} to extract feature map. Usually, this is taken directly from common architectures of classification task, such as VGG, ResNet, ResNeXt, MobileNet or DenseNet, and often pretrained on ImageNet.
	\item \textbf{Neck or Feature Pyramid} to extract and fuse feature from different layers of Backbone. This helps to detect objects at different scale, such as small object is detected at low level (but high resolution) layer, while large objects are detected on high level (but lower resolution) layer. 
	\item \textbf{Head} usually composes of two sub-networks to perform localization and classification. 
	\item \textbf{Loss}: Different works propose different type of loss function, so that optimization loss is as close as possible to the evaluation metrics, i.e. mean of Averange Precision (mAP) on different Itersection-over-Union (IoU). 
	\item \textbf{Post-Processing} to filter the predictions into final result. Typical steps include threshold prediction score and non-maxima-suppression to select the a single best from overlapped prediction boxes surrounding one object. 
\end{itemize}

\subsubsection{SOTA Methods and New Research Trending}
Among aforementioned components of object detection, Backbone and Neck network architecture, Loss functions and Post-processing steps can be generally applied to any approaches. However, each method proposes its own head and anchor setting, aiming to improve the accuracy and efficiency of Single Stage Object detection. In fact, anchor box is a fundamental component but has various designs. Overall, anchor setting has several limitations: 
\begin{itemize}
	\item Hyper-parameters, e.g size, aspect ratios and scales, need to be tuned to match with the target objects.
	\item Fixed hyper-parameters are not effective to handle object with various shape, especially smaller one.
	\item Anchor-boxed needs to be dense to cover wide range of object scale. It is used to believe that the denser anchor-box design, the higher accuracy detection. The excessive number of anchor-box leads to high computation IoU operator to identify anchor-boxes as positive samples (e.g. $IoU > 0.5$), and negative samples in training. Furthermore, using anchor boxes also lead to a cumbersome anchor-box encoder and decoder steps during training and inference, making the code complicated. 
	\item Data severe imbalance in training since negative samples outnumber positive ones by 1000 to 1. Although Focal loss \cite{Lin} can help to alleviate the problem, Focal Loss itself needs to be tuned. 
\end{itemize}  

Therefore, newest research shifts attention to remove the anchor-box step, and propose a new kind of framework name ``anchor-box free" approach. In general, anchor-box-free approach is designed to be simpler and more efficient than the current single-state approach. 

\begin{itemize}
	\item In fact, the first version of YOLO \cite{redmon2016you} does not use anchor-box. Instead, it divides an input image into a $S \times S$ grid. Each grid will predict $B$ bounding box $(x,y,w,h)$ and a confidence score $Pr(\rm{object})$ of how likely the box contains the object's center. Each grid cell also predicts $C$ conditional class probability $Pr(\rm{class_i|object})$. At inference phase, the class-specific confidence score is obtained by: $Pr(\rm{class|object})Pr(\rm{object})IOU_{pred}^{truth}$. However, since only box containing the object center are trained to predict object, YOLOv1 suffer low recall and high location error. Hence, YOLOv2 and YOLOv3 \cite{Redmon2017, Redmon2018} make use of the anchor-box design as well.
	\item CornerNet \cite{Law2018} is another anchor-free algorithm. It aims to detect a pair of corners of a bounding box, and then groups them to form the final detected bounding boxes. CornetNet uses a Hourglass network as backbone, and a network-branch to predict two sets of heatmaps, one to detect top-left corner and another for bottom-right corner. Each set of heatmaps is of dimension  $H \times W \times C$ , where channel $C$ is the number of categories. Each channel is a binary mask indicating the locations of the corners for a class, while the ground truth heatmap contain positive values at the locations of corners, diffused by a Gaussian distribution. 
	
	\begin{figure}[!h]
		\centering
		\begin{subfigure}{0.45\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./Fig/Framework/CornerNet-structure.png}	
			\caption{CornerNet structure. }
		\end{subfigure}%
		~
		\begin{subfigure}{.45\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./Fig/Framework/CornerNet-PredictModule.png}
			\caption{Corner-Pooling, Heatmap, Embedding and Offset branch.}
			
		\end{subfigure}
		\caption{CornerNet Detection Pipeline. Reprinted from \cite{Law2018}}
		\label{fig:CornerNet}
	\end{figure}
	
	To group corresponding top-left and bottom-right corners into a bounding box belonging to a single object, another network branch is used to predict embedding vector, such that distance between embeddings of two corners from the same object is small. Finally, to reduce the error due to down-sampling heatmap, another network-branch also predicts the offsets to slightly adjust the locations of the corners. \Fig{CornerNet} illustrate CornerNet structure. Unfortunately, CornerNet uses Hourglass backbone and multi-branch structure, which is not supported by our hardware. Furthermore, it requires grouping stage after keypoint detection, which significantly slowdown the algorithm.
	
	\item Duan et. al \cite{Duan2019a} proposed CenterNet-Triplet point, by adding a sub-module to detect center point upon the framework of CornetNet. The accuracy is improved however more computation cost needs to paid. Thus, it is not suitable for our speed demanding target. 
	
	\item Another work built upon CornerNet is CerterNet-SinglePoint proposed by Zhou et. al. \cite{Zhou2019}. The method aims to detect object'center from a keypoint heat map $\hat{Y}$ , which is of dimension $\frac{H}{R}\times \frac{W}{R} \times C$, where $C$ is the number of classes, and $R$ is the stride to downsample the image. Similar to CornerNet, they still have heatmap branch to detect keypoint, and offset-branch to adjust the location of center point. However, they only detect single center point, instead of a pair of corner points, thus avoid the complicated grouping step of embedding vector. In stead, a sub-branch is used to regress width and height of bounding box. In short, 3 sub-branchs networks are attached to the backbone to create key point heat map $\hat{Y}$, their offset $(\delta \hat{x}, \delta \hat{y})$ and size regression $(\hat{w},\hat{h})$, as illustrated in \fig{ObjAsPoint}. In addition, the DLA-34 network is modified and used as backbone, as illustrated in 
	
	\begin{figure}[!h]
		\centering
		\begin{subfigure}{0.65\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./Fig/Framework/ObjectAsPoint.png}
			\caption{Prediction of Head's sub-modules. }
		\end{subfigure}%
		\hspace{0.2in}
		\begin{subfigure}{.2\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./Fig/Framework/DLA-34.png}
			\caption{DLA-34 Backbone.}
			
		\end{subfigure}
		\centering
				
		\caption{Object As Points. Reprinted from \cite{Zhou2019}}
		\label{fig:ObjAsPoint}
	\end{figure}
	
	\item Among ``anchor-free" approaches,  FCOS \cite{DBLP:conf/iccv/abs-1904-01355} is the most successful. FCOS uses the similar structure of Retina, as shown in \Fig{FCOS}. However, it directly regresses the distance from all positive pixel to bounding box boundary $(l,r,t,b)$, and hence completely remove the need of anchor box. The most important setup used in FCOS is how to assign positive samples for training. A location $(x,y)$ is considered as a positive if it is inside a ground-truth bounding box, and the box label is assigned to class label of the location. If a pixel location falls into multiple bounding boxes, i.e. ambiguous sample, the bounding box with minimal area is used its regression target. Therefore, compared to Dense Anchor approach, such as RetinaNet, the number of positive samples is significantly larger since the positive samples in Retina is limited by anchor box IoU. The authors argue this characteristic makes training FCOS more accurate. Furthermore, at each pixel, we only predict C classes with 4 regressive parameters, while the corresponding values in RetinaNet is C class and $4k$, where $k$ is the number of anchor box at each location. Hence, FCOS is more sufficient and simpler. To suppress low-quality of bounding box, a single layer-branch is used in parallel with classification branch to predict ``center-ness" of a location. Given the regression target $(l^*,t^*,r^*,b^*)$, computed by the distance from the center to the ground truth bounding box, the target of centerness is defined as 
	\begin{equation}
	{\rm centerness^*} = \sqrt{\frac{\min(l^*,r^*)}{\max(l^*,r^*)} \frac{\min(t^*,b^*)}{\max(t^*,b^*)}}.
	\end{equation}  
	Note that, centerness approaches 1 if $l^*=r^*$ and $t^*=b^*$. 
	In testing phase, the confidence score is computed as product of classification score and predicted centerness. This, infact, is analogous to confidence score  $Pr(\rm{class|object})Pr(\rm{object})IOU_{pred}^{truth}$ of YOLO method mentioned above. 
	\begin{figure}[!h]
		\centering
		\begin{subfigure}{0.7\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./Fig/Framework/FCOS-framework.png}	
			\caption{FCOS . Reprinted from \cite{Tian2019}}
		\end{subfigure}
		\hspace{0.1in}
		\begin{subfigure}{.2\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./Fig/Framework/FCOS-centerness.png}
			\caption{Centerness Output. Reprinted from \cite{Tian2019}}
			
		\end{subfigure}
		\caption{FCOS Detection Pipeline}
		\label{fig:FCOS}
	\end{figure}

\end{itemize}

Observing that FCOS's detection quality is significantly better than Retina although their architectures are very similar, Zhang \textit{et al.} \cite{zhang2019bridging} investigates the main factors causing the performance gap. Their experiments reveal that the classification branch is the key for a high detection accuracy, while the regression one is less important. \textbf{They also challenge the preconception that dense anchors is indispensable by contradicting that using RetinaNet with only 1 anchor can get better detection quality than previous SOTA methods \Tab{cococompare}.} Therefore, they propose a new sampling strategy, called Adaptive Training Sample Selection (ATSS), which assign anchor more efficiently. Specifically, a bag of anchors is collected from multiple levels of the pyramid feature at a point. After that, Intersection over Union (IoU) between the ground truth and proposal anchors are computed and their mean and standard deviation of IoU are extracted. These metrics are used to set a IoU threshold for choosing the best matched proposal anchors to the examined ground truth. Doing so ensures about 20\% proposal anchors are assigned to a object, which solves the no-matched-anchor issue inside anchor-based method (Retinanet). 

\subsubsection{Comparision between SOTA methods for Object Detection}
\Tab{cococompare}\cite{zhang2019bridging} compares the performance of recently SOTA methods. It can be seen that using Retina with ATSS sampling strategy can outperforms the baseline Retinanet and FCOS by a large margin (up to 4.5 mAP) without any overhead in computation. Specifically, using the large backbone ResNeXt-101 it can achieve the top score, significantly better than the other with a large margin.

\pagebreak

\begin{table*}[!h]
\centering
\caption{Detection results on MS COCO {\tt test-dev} set, taken from \cite{zhang2019bridging}}
\vspace{-2mm}
\footnotesize \setlength{\tabcolsep}{9.5pt}
%\begin{threeparttable}
\begin{tabular}{|c|c|c|ccc|ccc|}
\hline
Method &Data &Backbone &AP &AP$_{50}$ &AP$_{75}$ &AP$_{\it S}$ &AP$_{\it M}$ &AP$_{\it L}$\\
\hline
\textit{anchor-based two-stage:} & & & & & & & & \\
MLKP \cite{DBLP:journals/corr/abs-1804-00428} &trainval35 &ResNet-101 &28.6 &52.4 &31.6 &10.8 &33.4 &45.1 \\
R-FCN \cite{DBLP:conf/nips/DaiLHS16} &trainval &ResNet-101 &29.9 &51.9 &- &10.8 &32.8 &45.0\\
CoupleNet \cite{DBLP:conf/iccv/abs-1708-02863} &trainval &ResNet-101 &34.4 &54.8 &37.2 &13.4 &38.1 &50.8 \\
TDM \cite{DBLP:journals/corr/ShrivastavaSMG16} &trainval &Inception-ResNet-v2-TDM &36.8 &57.7 &39.2 &16.2 &39.8 &52.1 \\
Hu et al. \cite{DBLP:journals/corr/abs-1711-11575} &trainval35k &ResNet-101 &39.0 &58.6 &42.9 &- &- &- \\
DeepRegionlets \cite{DBLP:conf/eccv/XuLWRBC18} &trainval35k &ResNet-101 &39.3 &59.8 &- &21.7 &43.7 &50.9 \\
FitnessNMS \cite{DBLP:journals/corr/abs-1711-00164} &trainval &DeNet-101 &39.5 &58.0 &42.6 &18.9 &43.5 &54.1 \\
Gu et al. \cite{DBLP:conf/eccv/GuHWWD18} &trainval35k &ResNet-101 &39.9 &63.1 &43.1 &22.2 &43.4 &51.6 \\
DetNet \cite{DBLP:journals/corr/abs-1804-06215} &trainval35k &DetNet-59 &40.3 &62.1 &43.8 &23.6 &42.6 &50.0 \\
umd\_det \cite{DBLP:conf/iccv/BodlaSCD17}  &trainval  &ResNet-101     &40.8 &62.4 &44.9 &23.0 &43.4 &53.2 \\
SOD-MTGAN \cite{DBLP:conf/eccv/BaiZDG18} &trainval35k &ResNet-101 &41.4 &63.2 &45.4 &24.7 &44.2 &52.6 \\
G-RMI \cite{DBLP:conf/cvpr/HuangRSZKFFWSG016} &trainval35k &Ensemble of Five Models &41.6 &61.9 &45.4 &23.9 &43.5 &54.9 \\
C-Mask RCNN \cite{DBLP:conf/eccv/ChenHT18} &trainval35k &ResNet-101 &42.0 &62.9 &46.4 &23.4 &44.7 &53.8 \\
Cascade R-CNN \cite{DBLP:conf/cvpr/abs-1712-00726} &trainval35k &ResNet-101 &42.8 &62.1 &46.3 &23.7 &45.5 &55.2 \\
Cascade RPN \cite{thangvurpn} &trainval35k &ResNet-50 &40.5 &59.3 &44.2 &22.5 &42.9 &51.5 \\
Revisiting RCNN \cite{DBLP:conf/eccv/ChengWSFXH18} &trainval35k &ResNet-101+ResNet-152 &43.1 &66.1 &47.3 &25.8 &45.9 &55.3 \\
SNIP \cite{DBLP:journals/corr/abs-1711-08189} &trainval35k &DPN-98 &45.7 &67.3 &51.1 &29.3 &48.8 &57.1 \\
\hline
\hline
\textit{anchor-based one-stage:} & & & & & & & & \\
YOLOv2 \cite{DBLP:conf/cvpr/RedmonF17} &trainval35k &DarkNet-19 &21.6 &44.0 &19.2 &5.0 &22.4 &35.5\\
SSD512$^*$ \cite{DBLP:conf/eccv/LiuAESRFB16} &trainval35k &VGG-16 &28.8 &48.5 &30.3 &10.9 &31.8 &43.5\\
STDN513 \cite{zhou2018scale}  &trainval &DenseNet-169 &31.8 &51.0 &33.6 &14.4 &36.1 &43.4\\
DES512 \cite{DBLP:journals/corr/abs-1712-00433}  &trainval35k &VGG-16 &32.8 &53.2 &34.5 &13.9 &36.2 &47.5 \\
DSSD513 \cite{DBLP:journals/corr/FuLRTB17} &trainval35k &ResNet-101 &33.2 &53.3 &35.2 &13.0 &35.4 &51.1 \\
RFB512-E \cite{DBLP:conf/eccv/LiuHW18}  &trainval35k  &VGG-16 &34.4 &55.7 &36.4 &17.6 &37.0 &47.6\\
DFP512 \cite{DBLP:conf/eccv/KongSHL18}  &trainval &ResNet-101 &34.6 &54.3 &37.3 &- &- &- \\
PFPNet-R512 \cite{DBLP:conf/eccv/KimKSKK18}  &trainval35k &VGG-16 &35.2 &57.6 &37.9 &18.7 &38.6 &45.9 \\
RefineDet512 \cite{DBLP:conf/cvpr/abs-1711-06897}  &trainval35k &ResNet-101 &36.4 &57.5 &39.5 &16.6 &39.9 &51.4 \\
RetinaNet \cite{DBLP:conf/iccv/LinPRK17} &trainval35k &ResNet-101 &39.1 &59.1 &42.3 &21.8 &42.7 &50.2 \\
\hline
\hline
\textit{anchor-free keypoint-based:} & & & & & & & & \\
ExtremeNet \cite{DBLP:conf/cvpr/ZhouZK19}   &trainval35k &Hourglass-104 &40.2 &55.5 &43.2 &20.4 &43.2 &53.1 \\
CornerNet \cite{DBLP:conf/eccv/LawD18}   &trainval35k &Hourglass-104 &40.5 &56.5 &43.1 &19.4 &42.7 &53.9 \\
CenterNet-HG \cite{DBLP:journals/corr/abs-1904-07850}   &trainval35k &Hourglass-104 &42.1 &61.1 &45.9 &24.1 &45.5 &52.8 \\
Grid R-CNN \cite{DBLP:conf/cvpr/LuLYLY19}   &trainval35k &ResNeXt-101 &43.2 &63.0 &46.6 &25.1 &46.5 &55.2 \\
CornerNet-Lite \cite{DBLP:journals/corr/abs-1904-08900}   &trainval35k &Hourglass-54 &43.2 &- &- &24.4 &44.6 &57.3 \\
CenterNet \cite{DBLP:journals/corr/abs-1904-08189}   &trainval35k &Hourglass-104 &44.9 &62.4 &48.1 &25.6 &47.4 &57.4 \\
RepPoints \cite{DBLP:journals/corr/abs-1904-11490}   &trainval35k &ResNet-101-DCN &45.0 &66.1 &49.0 &26.6 &48.6 &57.5 \\
\hline
\hline
\textit{anchor-free center-based:} & & & & & & & & \\
GA-RPN \cite{DBLP:conf/cvpr/WangCYLL19} &trainval35k &ResNet-50 &39.8 &59.2 &43.5 &21.8 &42.6 &50.7 \\
FoveaBox \cite{DBLP:journals/corr/abs-1904-03797} &trainval35k &ResNeXt-101 &42.1 &61.9 &45.2 &24.9 &46.8 &55.6 \\
FSAF \cite{DBLP:conf/cvpr/ZhuHS19} &trainval35k &ResNeXt-64x4d-101 &42.9 &63.8 &46.3 &26.6 &46.2 &52.7 \\
FCOS \cite{DBLP:conf/iccv/abs-1904-01355} &trainval35k &ResNeXt-64x4d-101 &43.2 &62.8 &46.6 &26.5 &46.2 &53.3 \\
\hline
\hline
\textit{adaptive sampling \cite{zhang2019bridging}:} & & & & & & & & \\
ATSS &trainval35k &ResNet-101 &43.6 &62.1 &47.4 &26.1 &47.0 &53.6 \\
ATSS &trainval35k &ResNeXt-32x8d-101 &45.1 &63.9 &49.1 &27.9 &48.2 &54.6 \\
ATSS &trainval35k &ResNeXt-64x4d-101 &45.6 &64.6 &49.7 &28.5 &48.9 &55.6 \\
ATSS &trainval35k &ResNet-101-DCN &46.3 &64.7 &50.4 &27.7 &49.8 &58.4 \\
ATSS &trainval35k &ResNeXt-32x8d-101-DCN &47.7 &66.6 &52.1 &29.3 &50.8 &59.7 \\
ATSS &trainval35k &ResNeXt-64x4d-101-DCN &47.7 &66.5 &51.9 &29.7 &50.8 &59.4 \\
ATSS (Multi-scale testing) &trainval35k &ResNeXt-32x8d-101-DCN &50.6 &68.6 &56.1 &\bf{33.6} &\bf{52.9} &62.2 \\
ATSS (Multi-scale testing) &trainval35k &ResNeXt-64x4d-101-DCN &\bf{50.7} &\bf{68.9} &\bf{56.3} &33.2 &\bf{52.9} &\bf{62.4} \\
\hline
\end{tabular}
\label{Tab:cococompare}
\end{table*}

